A Hybrid Transformer-Mamba Network for Single Image Deraining

Existing deraining Transformers employ self-attention mechanisms with fixed-range windows or along channel dimensions, limiting the exploitation of non-local receptive fields. In response to this issue, we introduce a novel dual-branch hybrid Transformer-Mamba network, denoted as TransMamba, aimed at effectively capturing long-range rain-related dependencies. Based on the prior of distinct spectral-domain features of rain degradation and background, we design a spectral-banded Transformer blocks on the first branch. Self-attention is executed within the combination of the spectral-domain channel dimension to improve the ability of modeling long-range dependencies. To enhance frequency-specific information, we present a spectral enhanced feed-forward module that aggregates features in the spectral domain. In the second branch, Mamba layers are equipped with cascaded bidirectional state space model modules to additionally capture the modeling of both local and global information. At each stage of both the encoder and decoder, we perform channel-wise concatenation of dual-branch features and achieve feature fusion through channel reduction, enabling more effective integration of the multi-scale information from the Transformer and Mamba branches. To better reconstruct innate signal-level relations within clean images, we also develop a spectral coherence loss. Extensive experiments on diverse datasets and real-world images demonstrate the superiority of our method compared against the state-of-the-art approaches.

==> sec/0_abstract_.tex <==
\begin{abstract}
%Transformer-based networks have made substantial advancements in the domain of single image deraining.
%, thanks to their proficiency in extracting extensive spatial information and modeling rain-induced degradation attributes. 
%However, the 
Existing deraining Transformers employ self-attention mechanisms with fixed-range windows or along channel dimensions, limiting the exploitation of non-local receptive fields. 
%
In response to this issue, we introduce a novel spectral-domain banding Transformer, denoted as SDBFormer, aimed at effectively capturing long-range rain-related dependencies. 
% Each spectral-domain token encodes a sinusoidal component decomposed from the global signal, thereby inherently implying long-range information of the original spatial representation. 
Spectral-domain tokens inherently imply long-range information of the original spatial representation. 
Additionally, we observe that the spectral bands, characterized by distinct frequencies, intrinsically separate the regions of rain streaks with repetitive patterns and the background featuring rich textures. 
% The bands of higher frequencies predominantly capture the intricacies of textured background regions, while those with lower frequencies distinctly portray the repetitive patterns associated with rain. 
% Triplet features of Query, Key and Value are converted into the spectral domain through the Fast Fourier Transform,
%and these tokens within the triplets are
We thus propose allocating varying degrees of attention to different spectral bands to adaptively filter rain streaks and recover background. 
% are thus categorized into distinct spectral bands according to a pre-computed mesh index. 
Self-attention is consequently executed within the combination of the spectral-domain channel dimension and spectral bands, to comprehensively capture both local information and long-range dependencies. 
%the categorization of 
% This process enables the comprehensive capture of both local information and long-range dependencies. 
%
To enhance frequency-specific information,
%of rain-related and background features, 
we present a spectral enhanced feed-forward module that aggregates features in the spectral domain. 
%
% Furthermore, we observe that the prevailing loss functions primarily emphasize pixel-wise proximity between predictions and targets, inadvertently neglecting their broader signal-level relationships. 
% To address this, we introduce a spectral coherence loss to measure the linear coherence between the recovered and target signals.
To enable the balance of the local and glabl modeling, we 
To better reconstruct innate signal-level relations within clean images, we also develop a spectral coherence loss.
%and compels the derained image to emulate the innate relation with the clean signal. 
Extensive experiments on diverse datasets and real-world images demonstrate the superiority of our method compared against the state-of-the-art approaches. 
We will release the codes and pre-trained models.
\end{abstract}

\begin{IEEEkeywords}
Single image deraining, Rain streak removal, Image restoration, Spectral domain
\end{IEEEkeywords}

==> sec/Z_biography.tex <==

% %-------------------------------------------------------------------------
% \newpage
% \section{Biography Section}
% If you have an EPS/PDF photo (graphicx package needed), extra braces are
%  needed around the contents of the optional argument to biography to prevent
%  the LaTeX parser from getting confused when it sees the complicated
%  $\backslash${\tt{includegraphics}} command within an optional argument. (You can create
%  your own custom macro containing the $\backslash${\tt{includegraphics}} command to make things
%  simpler here.)
 
% \vspace{11pt}

% \bf{If you include a photo:}
\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,trim={0 0.5cm 0 1.7cm},clip,keepaspectratio]{figs/biography/shangquan.JPG}}]{Shangquan Sun}
is currently a Ph.D. candidate at the Institute of Information Engineering, Chinese Academy of Sciences, Beijing, China, and the School of Cyber Security, University of Chinese Academy of Sciences, Beijing, China. His research interests include low-level image processing.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/biography/wenqi.png}}]{Wenqi Ren}
(Member, IEEE) received the Ph.D. degree from Tianjin University, Tianjin, China, in 2017. From 2015 to 2016, he was supported by the China Scholarship Council and working with Prof. Ming-Husan Yang as a joint-training Ph.D. Student with the Electrical Engineering and Computer Science Department, University of California at Merced. He is currently an Associate Professor with the School of Cyber Science and Technology, Shenzhen Campus of Sun Yat-sen University, Shenzhen, China. His research interests include image processing and related high-level vision problems.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/biography/rui.jpeg}}]{Rui Wang}
(Member, IEEE) received the bachelor's degree from Tsinghua University, China, in 2005, and the Ph.D. degree from Graduate University of Chinese Academy of Sciences, China, in 2011. Currently, she works in Institute of Information Engineering, Chinese Academy of Sciences, as a professor and doctoral supervisor. Her research interests include computer vision and artificial intelligence security..
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/biography/xiaochun.png}}]{Xiaochun Cao}
(Senior Member, IEEE) is a Professor and Dean of School of Cyber Science and Technology, Shenzhen Campus of Sun Yat-sen University. He received the B.E. and M.E. degrees both in computer science from Beihang University (BUAA), China, and the Ph.D. degree in computer science from the University of Central Florida, USA, with his dissertation nominated for the university level Outstanding Dissertation Award. After graduation, he spent about three years at ObjectVideo Inc. as a Research Scientist. From 2008 to 2012, he was a professor at Tianjin University. Before joining SYSU, he was a professor at Institute of Information Engineering, Chinese Academy of Sciences. He has authored and coauthored over 200 journal and conference papers. In 2004 and 2010, he was the recipients of the Piero Zamperoni best student paper award at the International Conference on Pattern Recognition. He is on the editorial boards of IEEE Transactions on Pattern Analysis and Machine Intelligence and IEEE Transactions on Image Processing, and was on the editorial boards of IEEE Transactions on Circuits and Systems for Video Technology and IEEE Transactions on Multimedia.  
\end{IEEEbiography}
% \vspace{11pt}

% \bf{If you will not include a photo:}\vspace{-33pt}
% \begin{IEEEbiographynophoto}{John Doe}
% Use $\backslash${\tt{begin\{IEEEbiographynophoto\}}} and the author name as the argument followed by the biography text.
% \end{IEEEbiographynophoto}

% %-------------------------------------------------------------------------

==> sec/fig_tex/ablation_rebuttal.tex <==
\begin{figure}[t]
  \centering
  \begin{minipage}{0.195\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
  \begin{annotationimage}{width=1\linewidth}{figs/ablation/input.png}
    \node[fill opacity=1,text=white] at (0.5,0.11) {\scriptsize Input};
    \end{annotationimage}
  \end{subfigure}
    \end{minipage}
  \hspace{-1.25mm}
  \centering
  \begin{minipage}{0.195\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
  \begin{annotationimage}{width=1\linewidth}{figs/ablation/exp1.png}
    \node[fill opacity=1,text=white] at (0.5,0.20) {\tiny Only low-freq.};
    \node[fill opacity=1,text=white] at (0.5,0.10) {\tiny (47.39/0.9912)};
    \end{annotationimage}
  \end{subfigure}
    \end{minipage}
  \hspace{-1.25mm}
  \centering
  \begin{minipage}{0.195\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
  \begin{annotationimage}{width=1\linewidth}{figs/ablation/exp2.png}
    \node[fill opacity=1,text=white] at (0.5,0.20) {\tiny Only high-freq.};
    \node[fill opacity=1,text=white] at (0.5,0.10) {\tiny (48.23/0.9919)};
    \end{annotationimage}
  \end{subfigure}
    \end{minipage}
  \hspace{-1.25mm}
  \centering
  \begin{minipage}{0.195\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
  \begin{annotationimage}{width=1\linewidth}{figs/ablation/ours.png}
    \node[fill opacity=1,text=white] at (0.5,0.20) {\tiny Ours};
    \node[fill opacity=1,text=white] at (0.5,0.10) {\tiny (48.91/0.9943)};
    \end{annotationimage}
  \end{subfigure}
    \end{minipage}
  \hspace{-1.25mm}
  \centering
  \begin{minipage}{0.195\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
  \begin{annotationimage}{width=1\linewidth}{figs/ablation/clean.png}
    \node[fill opacity=1,text=white] at (0.5,0.11) {\scriptsize Clean};
    \end{annotationimage}
  \end{subfigure}
    \end{minipage}
\vspace{-3.5mm}
  \caption{Extra ablation studies on SPA-Data with PSNR/SSIM.}
  \label{fig:ablation_rebuttal}
  \vspace{-3mm}
\end{figure}

==> sec/fig_tex/attn_map.tex <==
\begin{figure}[t]
  \centering
  \begin{minipage}{0.324\linewidth}
    \centering
  \begin{annotationimage}{trim=0 0 80 80,clip,width=1\linewidth}{figs/attn_map/input.jpeg}
    \node[fill opacity=1,text=white] at (0.5,0.11) {\scriptsize Input};
    \end{annotationimage}
    \end{minipage}
  \hspace{-1.55mm}
  \begin{minipage}{0.324\linewidth}
    \centering
    \begin{annotationimage}{trim=0 0 170 170,clip,width=1\linewidth}{figs/attn_map/1_7.jpeg}
    \node[fill opacity=1] at (0.5,0.11) {\scriptsize Before SBSA};
    \end{annotationimage}  
    \end{minipage}
  \hspace{-1.55mm}
  \begin{minipage}{0.324\linewidth}
    \centering
    \begin{annotationimage}{trim=0 0 80 80,clip,width=1\linewidth}{figs/attn_map/40_0.jpeg}
    \node[fill opacity=1] at (0.5,0.11) {\scriptsize $F_{1,1}$ in SBSA};
    \end{annotationimage}
    \end{minipage}
    
  \hspace{-1.55mm}
  \begin{minipage}{0.324\linewidth}
    \centering
    \begin{annotationimage}{trim=0 0 80 80,clip,width=1\linewidth}{figs/attn_map/3_1.jpeg}
    \node[fill opacity=1] at (0.5,0.11) {\scriptsize $F_{1,2}$ in SBSA};
    \end{annotationimage}
    \end{minipage}
  \hspace{-1.55mm}
  \begin{minipage}{0.324\linewidth}
    \centering
    \begin{annotationimage}{trim=0 0 80 80,clip,width=1\linewidth}{figs/attn_map/1_9.jpeg}
    \node[fill opacity=1] at (0.5,0.11) {\scriptsize $F_{2,1}$ in SBSA};
    \end{annotationimage}
    \end{minipage}
  \hspace{-1.55mm}
  \begin{minipage}{0.324\linewidth}
    \centering
    \begin{annotationimage}{trim=0 0 80 80,clip,width=1\linewidth}{figs/attn_map/40_5.jpeg}
    \node[fill opacity=1] at (0.5,0.11) {\scriptsize $F_{2,2}$ in SBSA};
    \end{annotationimage}
    \end{minipage}
  % \hspace{-1.55mm}
  % \begin{minipage}{0.324\linewidth}
  %   \centering
  % \begin{subfigure}{1\linewidth}
  %   \includegraphics[width=1\linewidth]{figs/bdd_coco/clean_00adbb3f-7757d4ea.jpeg}
  % \end{subfigure}
  %   \subcaption[]{\scriptsize Clean}
  %   \end{minipage}
  \caption{Attention map visualization. $F_{i,j}$ represents the map at $i$-th band and $j$-th channel. $F_{1,\{\cdot\}}$ focuses on background, while $F_{2,\{\cdot\}}$ focuses on rain streaks of different frequencies. Rain streaks and background are separated into two spectral bands.}
  \label{fig:attn}
\end{figure}

==> sec/fig_tex/cover.tex <==
\begin{figure}
  \centering
  \begin{minipage}{0.325\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/spa/rainy_SPA-Data_norain-941.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{figs/spa/rainy_SPA-Data_patch0_norain-941.png}
  \end{subfigure}
    \hspace{-1.5mm}
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{figs/spa/rainy_SPA-Data_patch2_norain-941.png}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.325\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/spa/IDT_SPA-Data_941.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{figs/spa/IDT_SPA-Data_patch0_941.png}
  \end{subfigure}
    \hspace{-1.5mm}
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{figs/spa/IDT_SPA-Data_patch2_941.png}
  \end{subfigure}
    \subcaption[]{IDT}
    \end{minipage}
  \hfill
  \begin{minipage}{0.325\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/spa/DRSformer_SPA-Data_941.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{figs/spa/DRSformer_SPA-Data_patch0_941.png}
  \end{subfigure}
    \hspace{-1.5mm}
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{figs/spa/DRSformer_SPA-Data_patch2_941.png}
  \end{subfigure}
    \subcaption[]{DRSformer}
    \end{minipage}
  
  \centering
  \begin{minipage}{0.325\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/spa/UDR_SPA-Data_norain-941.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{figs/spa/UDR_SPA-Data_patch0_norain-941.png}
  \end{subfigure}
    \hspace{-1.5mm}
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{figs/spa/UDR_SPA-Data_patch2_norain-941.png}
  \end{subfigure}
    \subcaption[]{\scriptsize UDR-S$^2$Former}
    \end{minipage}
  \hfill
  \begin{minipage}{0.325\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/spa/ours_SPA-Data_norain-941.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{figs/spa/ours_SPA-Data_patch0_norain-941.png}
  \end{subfigure}
    \hspace{-1.5mm}
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{figs/spa/ours_SPA-Data_patch2_norain-941.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hfill
  \begin{minipage}{0.325\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/spa/gt_SPA-Data_norain-941.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{figs/spa/gt_SPA-Data_patch0_norain-941.png}
  \end{subfigure}
    \hspace{-1.5mm}
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{figs/spa/gt_SPA-Data_patch2_norain-941.png}
  \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
  \caption{Visual comparisons among our method and the state-of-the-art Transformer deraining methods of real-world deraining on SPA-Data~\cite{wang2019spatial}. Our method produces the best deraining results}
  \label{fig:short}
\end{figure}

==> sec/fig_tex/desnow.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.240\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/input_winter_weather_06036.jpg}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.475\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/img_patch0_input_winter_weather_06036.jpg}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.475\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/img_patch1_input_winter_weather_06036.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.240\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/spdnet_winter_weather_06036.jpg}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.475\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/img_patch0_spdnet_winter_weather_06036.jpg}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.475\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/img_patch1_spdnet_winter_weather_06036.jpg}
  \end{subfigure}
    \subcaption[]{SPDNet~\cite{yi2021Structure}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.240\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/restormer_winter_weather_06036.jpg}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.475\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/img_patch0_restormer_winter_weather_06036.jpg}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.475\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/img_patch1_restormer_winter_weather_06036.jpg}
  \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.240\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/idt_winter_weather_06036.jpg}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.475\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/img_patch0_idt_winter_weather_06036.jpg}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.475\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/img_patch1_idt_winter_weather_06036.jpg}
  \end{subfigure}
    \subcaption[]{IDT~\cite{xiao2022image}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.240\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/drsformer_winter_weather_06036.jpg}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.475\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/img_patch0_drsformer_winter_weather_06036.jpg}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.475\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/img_patch1_drsformer_winter_weather_06036.jpg}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{chen2023learning}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.240\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/udr_winter_weather_06036.jpg}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.475\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/img_patch0_udr_winter_weather_06036.jpg}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.475\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/img_patch1_udr_winter_weather_06036.jpg}
  \end{subfigure}
    \subcaption[]{UDR-S$^2$Former~\cite{chen2023sparse}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.240\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/ours_winter_weather_06036.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.475\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/img_patch0_ours_winter_weather_06036.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.475\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/img_patch1_ours_winter_weather_06036.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hfill
  \begin{minipage}{0.240\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/gt_winter_weather_06036.jpg}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.475\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/img_patch0_gt_winter_weather_06036.jpg}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.475\linewidth}
    \includegraphics[width=1\linewidth]{figs/snow/img_patch1_gt_winter_weather_06036.jpg}
  \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
    % \vspace{-2mm}
  \caption{A visual comparison of desnowing by the deraining methods on Snow100K-L~\cite{liu2018desnownet}.}
  \label{fig:desnow}
  % \vspace{-2mm}
\end{figure*}

==> sec/fig_tex/did_ddn/ddn-1.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/rainy_DDN-Data_69.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/rainy_DDN-Data_patch0_69.jpg}
    \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DualGCN_DDN-Data_69.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DualGCN_DDN-Data_patch0_69.png}
    \end{subfigure}
    \subcaption[]{DualGCN}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/SPDNet_DDN-Data_69.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/SPDNet_DDN-Data_patch0_69.png}
    \end{subfigure}
    \subcaption[]{SPDNet}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/Restormer_DDN-Data_69.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/Restormer_DDN-Data_patch0_69.png}
    \end{subfigure}
    \subcaption[]{Restormer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/IDT_DDN-Data_69.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/IDT_DDN-Data_patch0_69.jpg}
    \end{subfigure}
    \subcaption[]{IDT}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DRSformer_DDN-Data_69.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DRSformer_DDN-Data_patch0_69.png}
    \end{subfigure}
    \subcaption[]{DRSformer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/UDR_DDN-Data_69.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/UDR_DDN-Data_patch0_69.png}
    \end{subfigure}
    \subcaption[]{\hspace{-0.5mm}\scriptsize UDR{\tiny -S$^2$}Former}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/ours_DDN-Data_69.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/ours_DDN-Data_patch0_69.png}
    \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/gt_DDN-Data_69.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/gt_DDN-Data_patch0_69.jpg}
    \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> sec/fig_tex/did_ddn/ddn-2.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/rainy_DDN-Data_70.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/rainy_DDN-Data_patch0_70.jpg}
    \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/rainy_DDN-Data_patch1_70.jpg}
    \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DualGCN_DDN-Data_70.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DualGCN_DDN-Data_patch0_70.png}
    \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DualGCN_DDN-Data_patch1_70.png}
    \end{subfigure}
    \subcaption[]{DualGCN~\cite{Fu2021RainSR}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/SPDNet_DDN-Data_70.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/SPDNet_DDN-Data_patch0_70.png}
    \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/SPDNet_DDN-Data_patch1_70.png}
    \end{subfigure}
    \subcaption[]{SPDNet~\cite{yi2021Structure}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/Restormer_DDN-Data_70.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/Restormer_DDN-Data_patch0_70.png}
    \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/Restormer_DDN-Data_patch1_70.png}
    \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/IDT_DDN-Data_70.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/IDT_DDN-Data_patch0_70.jpg}
    \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/IDT_DDN-Data_patch1_70.jpg}
    \end{subfigure}
    \subcaption[]{IDT~\cite{xiao2022image}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DRSformer_DDN-Data_70.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DRSformer_DDN-Data_patch0_70.png}
    \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DRSformer_DDN-Data_patch1_70.png}
    \end{subfigure}
    \subcaption[]{DRSformer~\cite{chen2023learning}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/UDR_DDN-Data_70.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/UDR_DDN-Data_patch0_70.png}
    \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/UDR_DDN-Data_patch1_70.png}
    \end{subfigure}
    \subcaption[]{UDR-S$^2$Former~\cite{chen2023sparse}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/ours_DDN-Data_70.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/ours_DDN-Data_patch0_70.png}
    \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/ours_DDN-Data_patch1_70.png}
    \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/gt_DDN-Data_70.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/gt_DDN-Data_patch0_70.jpg}
    \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/gt_DDN-Data_patch1_70.jpg}
    \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
  \caption{A visual comparison of deraining on DDN-Data~\cite{fu2017removing}.}
  \label{fig:ddn-2}
\end{figure*}

==> sec/fig_tex/did_ddn/ddn-3.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/rainy_DDN-Data_243.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/rainy_DDN-Data_patch0_243.jpg}
    \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DualGCN_DDN-Data_243.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DualGCN_DDN-Data_patch0_243.png}
    \end{subfigure}
    \subcaption[]{DualGCN}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/SPDNet_DDN-Data_243.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/SPDNet_DDN-Data_patch0_243.png}
    \end{subfigure}
    \subcaption[]{SPDNet}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/Restormer_DDN-Data_243.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/Restormer_DDN-Data_patch0_243.png}
    \end{subfigure}
    \subcaption[]{Restormer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/IDT_DDN-Data_243.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/IDT_DDN-Data_patch0_243.jpg}
    \end{subfigure}
    \subcaption[]{IDT}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DRSformer_DDN-Data_243.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DRSformer_DDN-Data_patch0_243.png}
    \end{subfigure}
    \subcaption[]{DRSformer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/UDR_DDN-Data_243.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/UDR_DDN-Data_patch0_243.png}
    \end{subfigure}
    \subcaption[]{\hspace{-0.5mm}\scriptsize UDR{\tiny -S$^2$}Former}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/ours_DDN-Data_243.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/ours_DDN-Data_patch0_243.png}
    \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/gt_DDN-Data_243.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/gt_DDN-Data_patch0_243.jpg}
    \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> sec/fig_tex/did_ddn/ddn-4.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/rainy_DDN-Data_285.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/rainy_DDN-Data_patch0_285.jpg}
    \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DualGCN_DDN-Data_285.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DualGCN_DDN-Data_patch0_285.png}
    \end{subfigure}
    \subcaption[]{DualGCN~\cite{Fu2021RainSR}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/SPDNet_DDN-Data_285.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/SPDNet_DDN-Data_patch0_285.png}
    \end{subfigure}
    \subcaption[]{SPDNet~\cite{yi2021Structure}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/Restormer_DDN-Data_285.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/Restormer_DDN-Data_patch0_285.png}
    \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/IDT_DDN-Data_285.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/IDT_DDN-Data_patch0_285.jpg}
    \end{subfigure}
    \subcaption[]{IDT~\cite{xiao2022image}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DRSformer_DDN-Data_285.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DRSformer_DDN-Data_patch0_285.png}
    \end{subfigure}
    \subcaption[]{DRSformer~\cite{chen2023learning}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/UDR_DDN-Data_285.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/UDR_DDN-Data_patch0_285.png}
    \end{subfigure}
    \subcaption[]{UDR-S$^2$Former~\cite{chen2023sparse}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/ours_DDN-Data_285.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/ours_DDN-Data_patch0_285.png}
    \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/gt_DDN-Data_285.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/gt_DDN-Data_patch0_285.jpg}
    \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
  \caption{A visual comparison of deraining on DDN-Data~\cite{fu2017removing}.}
  \label{fig:ddn-4}
\end{figure*}

==> sec/fig_tex/did_ddn/ddn-5.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/rainy_DDN-Data_292.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/rainy_DDN-Data_patch0_292.jpg}
    \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DualGCN_DDN-Data_292.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DualGCN_DDN-Data_patch0_292.png}
    \end{subfigure}
    \subcaption[]{DualGCN}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/SPDNet_DDN-Data_292.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/SPDNet_DDN-Data_patch0_292.png}
    \end{subfigure}
    \subcaption[]{SPDNet}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/Restormer_DDN-Data_292.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/Restormer_DDN-Data_patch0_292.png}
    \end{subfigure}
    \subcaption[]{Restormer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/IDT_DDN-Data_292.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/IDT_DDN-Data_patch0_292.jpg}
    \end{subfigure}
    \subcaption[]{IDT}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DRSformer_DDN-Data_292.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DRSformer_DDN-Data_patch0_292.png}
    \end{subfigure}
    \subcaption[]{DRSformer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/UDR_DDN-Data_292.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/UDR_DDN-Data_patch0_292.png}
    \end{subfigure}
    \subcaption[]{\hspace{-0.5mm}\scriptsize UDR{\tiny -S$^2$}Former}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/ours_DDN-Data_292.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/ours_DDN-Data_patch0_292.png}
    \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/gt_DDN-Data_292.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/gt_DDN-Data_patch0_292.jpg}
    \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> sec/fig_tex/did_ddn/ddn-6.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/rainy_DDN-Data_346.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/rainy_DDN-Data_patch0_346.jpg}
    \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DualGCN_DDN-Data_346.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DualGCN_DDN-Data_patch0_346.png}
    \end{subfigure}
    \subcaption[]{DualGCN}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/SPDNet_DDN-Data_346.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/SPDNet_DDN-Data_patch0_346.png}
    \end{subfigure}
    \subcaption[]{SPDNet}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/Restormer_DDN-Data_346.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/Restormer_DDN-Data_patch0_346.png}
    \end{subfigure}
    \subcaption[]{Restormer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/IDT_DDN-Data_346.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/IDT_DDN-Data_patch0_346.jpg}
    \end{subfigure}
    \subcaption[]{IDT}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DRSformer_DDN-Data_346.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/DRSformer_DDN-Data_patch0_346.png}
    \end{subfigure}
    \subcaption[]{DRSformer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/UDR_DDN-Data_346.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/UDR_DDN-Data_patch0_346.png}
    \end{subfigure}
    \subcaption[]{\hspace{-0.5mm}\scriptsize UDR{\tiny -S$^2$}Former}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/ours_DDN-Data_346.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/ours_DDN-Data_patch0_346.png}
    \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/gt_DDN-Data_346.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/ddn/gt_DDN-Data_patch0_346.jpg}
    \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> sec/fig_tex/did_ddn/did-1.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0mm 30mm 0mm 5mm,clip,width=1\linewidth]{figs/did/rainy_DID-Data_14.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/rainy_DID-Data_patch0_14.jpg}
    \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0mm 30mm 0mm 5mm,clip,width=1\linewidth]{figs/did/DualGCN_DID-Data_14.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/DualGCN_DID-Data_patch0_14.png}
    \end{subfigure}
    \subcaption[]{DualGCN~\cite{Fu2021RainSR}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0mm 30mm 0mm 5mm,clip,width=1\linewidth]{figs/did/SPDNet_DID-Data_14.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/SPDNet_DID-Data_patch0_14.png}
    \end{subfigure}
    \subcaption[]{SPDNet~\cite{yi2021Structure}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0mm 30mm 0mm 5mm,clip,width=1\linewidth]{figs/did/Restormer_DID-Data_14.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/Restormer_DID-Data_patch0_14.png}
    \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0mm 30mm 0mm 5mm,clip,width=1\linewidth]{figs/did/IDT_DID-Data_14.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/IDT_DID-Data_patch0_14.jpg}
    \end{subfigure}
    \subcaption[]{IDT~\cite{xiao2022image}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0mm 30mm 0mm 5mm,clip,width=1\linewidth]{figs/did/DRSformer_DID-Data_14.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/DRSformer_DID-Data_patch0_14.png}
    \end{subfigure}
    \subcaption[]{DRSformer~\cite{chen2023learning}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0mm 30mm 0mm 5mm,clip,width=1\linewidth]{figs/did/UDR_DID-Data_14.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/UDR_DID-Data_patch0_14.png}
    \end{subfigure}
    \subcaption[]{UDR-S$^2$Former~\cite{chen2023sparse}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0mm 30mm 0mm 5mm,clip,width=1\linewidth]{figs/did/ours_DID-Data_14.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/ours_DID-Data_patch0_14.png}
    \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0mm 30mm 0mm 5mm,clip,width=1\linewidth]{figs/did/gt_DID-Data_14.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/gt_DID-Data_patch0_14.jpg}
    \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
    \vspace{-3mm}
  \caption{A visual comparison of deraining on DID-Data~\cite{zhang2018density}.}
  \label{fig:did-1}
\end{figure*}

==> sec/fig_tex/did_ddn/did-2.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0mm 5mm 0mm 5mm,clip,width=1\linewidth]{figs/did/rainy_DID-Data_20.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/rainy_DID-Data_patch0_20.jpg}
    \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0mm 5mm 0mm 5mm,clip,width=1\linewidth]{figs/did/DualGCN_DID-Data_20.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/DualGCN_DID-Data_patch0_20.png}
    \end{subfigure}
    \subcaption[]{DualGCN~\cite{Fu2021RainSR}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0mm 5mm 0mm 5mm,clip,width=1\linewidth]{figs/did/SPDNet_DID-Data_20.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/SPDNet_DID-Data_patch0_20.png}
    \end{subfigure}
    \subcaption[]{SPDNet~\cite{yi2021Structure}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0mm 5mm 0mm 5mm,clip,width=1\linewidth]{figs/did/Restormer_DID-Data_20.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/Restormer_DID-Data_patch0_20.png}
    \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0mm 5mm 0mm 5mm,clip,width=1\linewidth]{figs/did/IDT_DID-Data_20.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/IDT_DID-Data_patch0_20.jpg}
    \end{subfigure}
    \subcaption[]{IDT~\cite{xiao2022image}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0mm 5mm 0mm 5mm,clip,width=1\linewidth]{figs/did/DRSformer_DID-Data_20.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/DRSformer_DID-Data_patch0_20.png}
    \end{subfigure}
    \subcaption[]{DRSformer~\cite{chen2023learning}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0mm 5mm 0mm 5mm,clip,width=1\linewidth]{figs/did/UDR_DID-Data_20.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/UDR_DID-Data_patch0_20.png}
    \end{subfigure}
    \subcaption[]{UDR-S$^2$Former~\cite{chen2023sparse}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0mm 5mm 0mm 5mm,clip,width=1\linewidth]{figs/did/ours_DID-Data_20.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/ours_DID-Data_patch0_20.png}
    \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0mm 5mm 0mm 5mm,clip,width=1\linewidth]{figs/did/gt_DID-Data_20.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/gt_DID-Data_patch0_20.jpg}
    \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
    \vspace{-3mm}
  \caption{A visual comparison of deraining on DID-Data~\cite{zhang2018density}.}
  \label{fig:did-2}
\end{figure*}

==> sec/fig_tex/did_ddn/did-3.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/rainy_DID-Data_24.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/rainy_DID-Data_patch0_24.jpg}
    \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/DualGCN_DID-Data_24.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/DualGCN_DID-Data_patch0_24.png}
    \end{subfigure}
    \subcaption[]{DualGCN}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/SPDNet_DID-Data_24.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/SPDNet_DID-Data_patch0_24.png}
    \end{subfigure}
    \subcaption[]{SPDNet}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/Restormer_DID-Data_24.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/Restormer_DID-Data_patch0_24.png}
    \end{subfigure}
    \subcaption[]{Restormer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/IDT_DID-Data_24.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/IDT_DID-Data_patch0_24.jpg}
    \end{subfigure}
    \subcaption[]{IDT}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/DRSformer_DID-Data_24.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/DRSformer_DID-Data_patch0_24.png}
    \end{subfigure}
    \subcaption[]{DRSformer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/UDR_DID-Data_24.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/UDR_DID-Data_patch0_24.png}
    \end{subfigure}
    \subcaption[]{UDR-S$^2$Former}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/ours_DID-Data_24.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/ours_DID-Data_patch0_24.png}
    \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/gt_DID-Data_24.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/gt_DID-Data_patch0_24.jpg}
    \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> sec/fig_tex/did_ddn/did-4.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/rainy_DID-Data_96.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/rainy_DID-Data_patch0_96.jpg}
    \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/DualGCN_DID-Data_96.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/DualGCN_DID-Data_patch0_96.png}
    \end{subfigure}
    \subcaption[]{DualGCN}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/SPDNet_DID-Data_96.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/SPDNet_DID-Data_patch0_96.png}
    \end{subfigure}
    \subcaption[]{SPDNet}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/Restormer_DID-Data_96.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/Restormer_DID-Data_patch0_96.png}
    \end{subfigure}
    \subcaption[]{Restormer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/IDT_DID-Data_96.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/IDT_DID-Data_patch0_96.jpg}
    \end{subfigure}
    \subcaption[]{IDT}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/DRSformer_DID-Data_96.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/DRSformer_DID-Data_patch0_96.png}
    \end{subfigure}
    \subcaption[]{DRSformer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/UDR_DID-Data_96.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/UDR_DID-Data_patch0_96.png}
    \end{subfigure}
    \subcaption[]{UDR-S$^2$Former}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/ours_DID-Data_96.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/ours_DID-Data_patch0_96.png}
    \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/gt_DID-Data_96.jpg}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/did/gt_DID-Data_patch0_96.jpg}
    \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> sec/fig_tex/rain200/rain200H-1.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 15mm 0 50mm,clip,width=1\linewidth]{figs/rain200H/rainy_Rain200H_159.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/rainy_Rain200H_patch0_159.png}
    \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 15mm 0 50mm,clip,width=1\linewidth]{figs/rain200H/DualGCN_Rain200H_159.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/DualGCN_Rain200H_patch0_159.png}
    \end{subfigure}
    \subcaption[]{DualGCN~\cite{Fu2021RainSR}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 15mm 0 50mm,clip,width=1\linewidth]{figs/rain200H/SPDNet_Rain200H_159.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/SPDNet_Rain200H_patch0_159.png}
    \end{subfigure}
    \subcaption[]{SPDNet~\cite{yi2021Structure}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 15mm 0 50mm,clip,width=1\linewidth]{figs/rain200H/Restormer_Rain200H_159.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/Restormer_Rain200H_patch0_159.png}
    \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 15mm 0 50mm,clip,width=1\linewidth]{figs/rain200H/IDT_Rain200H_159.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/IDT_Rain200H_patch0_159.png}
    \end{subfigure}
    \subcaption[]{IDT~\cite{xiao2022image}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 15mm 0 50mm,clip,width=1\linewidth]{figs/rain200H/DRSformer_Rain200H_159.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/DRSformer_Rain200H_patch0_159.png}
    \end{subfigure}
    \subcaption[]{DRSformer~\cite{chen2023learning}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 15mm 0 50mm,clip,width=1\linewidth]{figs/rain200H/UDR_Rain200H_159.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/UDR_Rain200H_patch0_159.png}
    \end{subfigure}
    \subcaption[]{UDR-S$^2$Former~\cite{chen2023sparse}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 15mm 0 50mm,clip,width=1\linewidth]{figs/rain200H/ours_Rain200H_159.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/ours_Rain200H_patch0_159.png}
    \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 15mm 0 50mm,clip,width=1\linewidth]{figs/rain200H/gt_Rain200H_159.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/gt_Rain200H_patch0_159.png}
    \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
    \vspace{-3mm}
  \caption{A visual comparison of deraining on Rain200H~\cite{yang2017deep}.}
  \label{fig:supple_rain200h-1}
\end{figure*}

==> sec/fig_tex/rain200/rain200H-2.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 0mm 0 65mm,clip,width=1\linewidth]{figs/rain200H/rainy_Rain200H_178.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/rainy_Rain200H_patch0_178.png}
    \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 0mm 0 65mm,clip,width=1\linewidth]{figs/rain200H/DualGCN_Rain200H_178.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/DualGCN_Rain200H_patch0_178.png}
    \end{subfigure}
    \subcaption[]{DualGCN~\cite{Fu2021RainSR}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 0mm 0 65mm,clip,width=1\linewidth]{figs/rain200H/SPDNet_Rain200H_178.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/SPDNet_Rain200H_patch0_178.png}
    \end{subfigure}
    \subcaption[]{SPDNet~\cite{yi2021Structure}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 0mm 0 65mm,clip,width=1\linewidth]{figs/rain200H/Restormer_Rain200H_178.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/Restormer_Rain200H_patch0_178.png}
    \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 0mm 0 65mm,clip,width=1\linewidth]{figs/rain200H/IDT_Rain200H_178.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/IDT_Rain200H_patch0_178.png}
    \end{subfigure}
    \subcaption[]{IDT~\cite{xiao2022image}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 0mm 0 65mm,clip,width=1\linewidth]{figs/rain200H/DRSformer_Rain200H_178.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/DRSformer_Rain200H_patch0_178.png}
    \end{subfigure}
    \subcaption[]{DRSformer~\cite{chen2023learning}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 0mm 0 65mm,clip,width=1\linewidth]{figs/rain200H/UDR_Rain200H_178.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/UDR_Rain200H_patch0_178.png}
    \end{subfigure}
    \subcaption[]{UDR-S$^2$Former~\cite{chen2023sparse}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 0mm 0 65mm,clip,width=1\linewidth]{figs/rain200H/ours_Rain200H_178.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/ours_Rain200H_patch0_178.png}
    \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 0mm 0 65mm,clip,width=1\linewidth]{figs/rain200H/gt_Rain200H_178.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/gt_Rain200H_patch0_178.png}
    \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
    \vspace{-3mm}
  \caption{A visual comparison of deraining on Rain200H~\cite{yang2017deep}.}
  \label{fig:supple_rain200h-2}
\end{figure*}

==> sec/fig_tex/rain200/rain200H-3.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/rainy_Rain200H_183.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/rainy_Rain200H_patch0_183.png}
    \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/DualGCN_Rain200H_183.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/DualGCN_Rain200H_patch0_183.png}
    \end{subfigure}
    \subcaption[]{DualGCN~\cite{Fu2021RainSR}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/SPDNet_Rain200H_183.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/SPDNet_Rain200H_patch0_183.png}
    \end{subfigure}
    \subcaption[]{SPDNet~\cite{yi2021Structure}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/Restormer_Rain200H_183.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/Restormer_Rain200H_patch0_183.png}
    \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/IDT_Rain200H_183.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/IDT_Rain200H_patch0_183.png}
    \end{subfigure}
    \subcaption[]{IDT~\cite{xiao2022image}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/DRSformer_Rain200H_183.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/DRSformer_Rain200H_patch0_183.png}
    \end{subfigure}
    \subcaption[]{DRSformer~\cite{chen2023learning}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/UDR_Rain200H_183.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/UDR_Rain200H_patch0_183.png}
    \end{subfigure}
    \subcaption[]{UDR-S$^2$Former~\cite{chen2023sparse}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/ours_Rain200H_183.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/ours_Rain200H_patch0_183.png}
    \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/gt_Rain200H_183.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/gt_Rain200H_patch0_183.png}
    \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
    \vspace{-3mm}
  \caption{A visual comparison of deraining on Rain200H~\cite{yang2017deep}.}
  \label{fig:supple_rain200h-3}
\end{figure*}

==> sec/fig_tex/rain200/rain200H-4.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/rainy_Rain200H_199.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/rainy_Rain200H_patch0_199.png}
    \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/rainy_Rain200H_patch1_199.png}
    \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/DualGCN_Rain200H_199.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/DualGCN_Rain200H_patch0_199.png}
    \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/DualGCN_Rain200H_patch1_199.png}
    \end{subfigure}
    \subcaption[]{DualGCN~\cite{Fu2021RainSR}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/SPDNet_Rain200H_199.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/SPDNet_Rain200H_patch0_199.png}
    \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/SPDNet_Rain200H_patch1_199.png}
    \end{subfigure}
    \subcaption[]{SPDNet~\cite{yi2021Structure}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/Restormer_Rain200H_199.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/Restormer_Rain200H_patch0_199.png}
    \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/Restormer_Rain200H_patch1_199.png}
    \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/IDT_Rain200H_199.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/IDT_Rain200H_patch0_199.png}
    \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/IDT_Rain200H_patch1_199.png}
    \end{subfigure}
    \subcaption[]{IDT~\cite{xiao2022image}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/DRSformer_Rain200H_199.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/DRSformer_Rain200H_patch0_199.png}
    \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/DRSformer_Rain200H_patch1_199.png}
    \end{subfigure}
    \subcaption[]{DRSformer~\cite{chen2023learning}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/UDR_Rain200H_199.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/UDR_Rain200H_patch0_199.png}
    \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/UDR_Rain200H_patch1_199.png}
    \end{subfigure}
    \subcaption[]{UDR-S$^2$Former~\cite{chen2023sparse}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/ours_Rain200H_199.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/ours_Rain200H_patch0_199.png}
    \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/ours_Rain200H_patch1_199.png}
    \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hfill
  \begin{minipage}{0.327\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/gt_Rain200H_199.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/gt_Rain200H_patch0_199.png}
    \end{subfigure}
    \hfill
     \begin{subfigure}{0.485\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/gt_Rain200H_patch1_199.png}
    \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
    \vspace{-3mm}
  \caption{A visual comparison of deraining on Rain200H~\cite{yang2017deep}.}
  \label{fig:supple_rain200h-4}
  \vspace{-3mm}
\end{figure*}

==> sec/fig_tex/rain200/rain200L-1.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/rainy_Rain200L_89.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/rainy_Rain200L_patch0_89.png}
    \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/DualGCN_Rain200L_89.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/DualGCN_Rain200L_patch0_89.png}
    \end{subfigure}
    \subcaption[]{DualGCN}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/SPDNet_Rain200L_89.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/SPDNet_Rain200L_patch0_89.png}
    \end{subfigure}
    \subcaption[]{SPDNet}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/Restormer_Rain200L_89.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/Restormer_Rain200L_patch0_89.png}
    \end{subfigure}
    \subcaption[]{Restormer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/IDT_Rain200L_89.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/IDT_Rain200L_patch0_89.png}
    \end{subfigure}
    \subcaption[]{IDT}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/DRSformer_Rain200L_89.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/DRSformer_Rain200L_patch0_89.png}
    \end{subfigure}
    \subcaption[]{DRSformer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/UDR_Rain200L_89.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/UDR_Rain200L_patch0_89.png}
    \end{subfigure}
    \subcaption[]{\hspace{-0.5mm}\scriptsize UDR{\tiny -S$^2$}Former}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/ours_Rain200L_89.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/ours_Rain200L_patch0_89.png}
    \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/gt_Rain200L_89.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/gt_Rain200L_patch0_89.png}
    \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
  \caption{Visual comparisons of deraining on Rain200L (1st row) and Rain200H (2nd row) datasets~\cite{yang2017deep}. Please zoom in for a better view.}
  \label{fig:short}
\end{figure*}

==> sec/fig_tex/rain200/rain200L-2.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/rainy_Rain200L_137.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/rainy_Rain200L_patch0_137.png}
    \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/DualGCN_Rain200L_137.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/DualGCN_Rain200L_patch0_137.png}
    \end{subfigure}
    \subcaption[]{DualGCN}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/SPDNet_Rain200L_137.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/SPDNet_Rain200L_patch0_137.png}
    \end{subfigure}
    \subcaption[]{SPDNet}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/Restormer_Rain200L_137.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/Restormer_Rain200L_patch0_137.png}
    \end{subfigure}
    \subcaption[]{Restormer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/IDT_Rain200L_137.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/IDT_Rain200L_patch0_137.png}
    \end{subfigure}
    \subcaption[]{IDT}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/DRSformer_Rain200L_137.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/DRSformer_Rain200L_patch0_137.png}
    \end{subfigure}
    \subcaption[]{DRSformer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/UDR_Rain200L_137.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/UDR_Rain200L_patch0_137.png}
    \end{subfigure}
    \subcaption[]{\hspace{-0.5mm}\scriptsize UDR{\tiny -S$^2$}Former}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/ours_Rain200L_137.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/ours_Rain200L_patch0_137.png}
    \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hfill
  \begin{minipage}{0.107\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/gt_Rain200L_137.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200L/gt_Rain200L_patch0_137.png}
    \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> sec/fig_tex/rain200/rain200h_supple.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.120\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/rainy_Rain200H_199.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.488\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/rainy_Rain200H_patch0_199.png}
    \end{subfigure}
    \hspace{-1.3mm}
     \begin{subfigure}{0.488\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/rainy_Rain200H_patch1_199.png}
    \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/rainy_Rain200H_183.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/rainy_Rain200H_patch0_183.png}
    \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  % \hfill
  % \begin{minipage}{0.120\linewidth}
  %   \centering
  % \begin{subfigure}{1\linewidth}
  %   \includegraphics[width=1\linewidth]{figs/rain200H/DualGCN_Rain200H_199.png}
  % \end{subfigure}
  %   \hfill
  %    \begin{subfigure}{1\linewidth}
  %   \includegraphics[width=1\linewidth]{figs/rain200H/DualGCN_Rain200H_patch0_199.png}
  %   \end{subfigure}
  %   \hfill
  % \begin{subfigure}{1\linewidth}
  %   \includegraphics[width=1\linewidth]{figs/rain200H/DualGCN_Rain200H_183.png}
  % \end{subfigure}
  %   \hfill
  %    \begin{subfigure}{1\linewidth}
  %   \includegraphics[width=1\linewidth]{figs/rain200H/DualGCN_Rain200H_patch0_183.png}
  %   \end{subfigure}
  %   \subcaption[]{DualGCN}
  %   \end{minipage}
  \hfill
  \begin{minipage}{0.120\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/SPDNet_Rain200H_199.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.488\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/SPDNet_Rain200H_patch0_199.png}
    \end{subfigure}
    \hspace{-1.3mm}
     \begin{subfigure}{0.488\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/SPDNet_Rain200H_patch1_199.png}
    \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/SPDNet_Rain200H_183.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/SPDNet_Rain200H_patch0_183.png}
    \end{subfigure}
    \subcaption[]{SPDNet}
    \end{minipage}
  \hfill
  \begin{minipage}{0.120\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/Restormer_Rain200H_199.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.488\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/Restormer_Rain200H_patch0_199.png}
    \end{subfigure}
    \hspace{-1.3mm}
     \begin{subfigure}{0.488\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/Restormer_Rain200H_patch1_199.png}
    \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/Restormer_Rain200H_183.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/Restormer_Rain200H_patch0_183.png}
    \end{subfigure}
    \subcaption[]{Restormer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.120\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/IDT_Rain200H_199.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.488\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/IDT_Rain200H_patch0_199.png}
    \end{subfigure}
    \hspace{-1.3mm}
     \begin{subfigure}{0.488\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/IDT_Rain200H_patch1_199.png}
    \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/IDT_Rain200H_183.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/IDT_Rain200H_patch0_183.png}
    \end{subfigure}
    \subcaption[]{IDT}
    \end{minipage}
  \hfill
  \begin{minipage}{0.120\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/DRSformer_Rain200H_199.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.488\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/DRSformer_Rain200H_patch0_199.png}
    \end{subfigure}
    \hspace{-1.3mm}
     \begin{subfigure}{0.488\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/DRSformer_Rain200H_patch1_199.png}
    \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/DRSformer_Rain200H_183.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/DRSformer_Rain200H_patch0_183.png}
    \end{subfigure}
    \subcaption[]{DRSformer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.120\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/UDR_Rain200H_199.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.488\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/UDR_Rain200H_patch0_199.png}
    \end{subfigure}
    \hspace{-1.3mm}
     \begin{subfigure}{0.488\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/UDR_Rain200H_patch1_199.png}
    \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/UDR_Rain200H_183.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/UDR_Rain200H_patch0_183.png}
    \end{subfigure}
    \subcaption[]{\scriptsize UDR-S$^2$Former}
    \end{minipage}
  \hfill
  \begin{minipage}{0.120\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/ours_Rain200H_199.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.488\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/ours_Rain200H_patch0_199.png}
    \end{subfigure}
    \hspace{-1.3mm}
     \begin{subfigure}{0.488\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/ours_Rain200H_patch1_199.png}
    \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/ours_Rain200H_183.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/ours_Rain200H_patch0_183.png}
    \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hfill
  \begin{minipage}{0.120\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/gt_Rain200H_199.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{0.488\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/gt_Rain200H_patch0_199.png}
    \end{subfigure}
    \hspace{-1.3mm}
     \begin{subfigure}{0.488\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/gt_Rain200H_patch1_199.png}
    \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/gt_Rain200H_183.png}
  \end{subfigure}
    \hfill
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/rain200H/gt_Rain200H_patch0_183.png}
    \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
    \vspace{-3mm}
  \caption{Visual comparisons of deraining on Rain200H~\cite{yang2017deep}. Please zoom in for a better view.}
  \label{fig:rain200H_supple}
  \vspace{-3mm}
\end{figure*}

==> sec/fig_tex/real/real-2.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/rainy_124.jpg}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/rainy_106.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/spdnet_124.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/spdnet_106.png}
  \end{subfigure}
    \subcaption[]{SPDNet}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/restormer_124.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/restormer_106.png}
  \end{subfigure}
    \subcaption[]{Restormer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/idt_124.jpg}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/idt_106.jpg}
  \end{subfigure}
    \subcaption[]{IDT}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/drsformer_124.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/drsformer_106.png}
  \end{subfigure}
    \subcaption[]{DRSformer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/udr_124.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/udr_106.png}
  \end{subfigure}
    \subcaption[]{\scriptsize UDR-S$^2$Former}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/ours_124.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/ours_106.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \caption{Visual comparisons of deraining on two samples from Internet-Data~\cite{wang2019spatial}. Please zoom in for a better view.}
  \label{fig:short}
\end{figure*}

==> sec/fig_tex/real/real-3.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/rainy_101.jpg}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/rainy_91.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/spdnet_101.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/spdnet_91.png}
  \end{subfigure}
    \subcaption[]{SPDNet}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/restormer_101.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/restormer_91.png}
  \end{subfigure}
    \subcaption[]{Restormer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/idt_101.jpg}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/idt_91.jpg}
  \end{subfigure}
    \subcaption[]{IDT}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/drsformer_101.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/drsformer_91.png}
  \end{subfigure}
    \subcaption[]{DRSformer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/udr_101.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/udr_91.png}
  \end{subfigure}
    \subcaption[]{\scriptsize UDR-S$^2$Former}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/ours_101.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/ours_91.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \caption{Visual comparisons of deraining on two samples from Internet-Data~\cite{wang2019spatial}. Please zoom in for a better view.}
  \label{fig:short}
\end{figure*}

==> sec/fig_tex/real/real-4.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/rainy_89.jpg}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/rainy_69.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/spdnet_89.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/spdnet_69.png}
  \end{subfigure}
    \subcaption[]{SPDNet}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/restormer_89.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/restormer_69.png}
  \end{subfigure}
    \subcaption[]{Restormer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/idt_89.jpg}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/idt_69.jpg}
  \end{subfigure}
    \subcaption[]{IDT}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/drsformer_89.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/drsformer_69.png}
  \end{subfigure}
    \subcaption[]{DRSformer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/udr_89.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/udr_69.png}
  \end{subfigure}
    \subcaption[]{\scriptsize UDR-S$^2$Former}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/ours_89.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/ours_69.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \caption{Visual comparisons of deraining on two samples from Internet-Data~\cite{wang2019spatial}. Please zoom in for a better view.}
  \label{fig:short}
\end{figure*}

==> sec/fig_tex/real/real-5.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/rainy_66.jpg}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/rainy_133.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/spdnet_66.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/spdnet_133.png}
  \end{subfigure}
    \subcaption[]{SPDNet}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/restormer_66.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/restormer_133.png}
  \end{subfigure}
    \subcaption[]{Restormer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/idt_66.jpg}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/idt_133.jpg}
  \end{subfigure}
    \subcaption[]{IDT}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/drsformer_66.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/drsformer_133.png}
  \end{subfigure}
    \subcaption[]{DRSformer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/udr_66.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/udr_133.png}
  \end{subfigure}
    \subcaption[]{\scriptsize UDR-S$^2$Former}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/ours_66.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/ours_133.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \caption{Visual comparisons of deraining on two samples from Internet-Data~\cite{wang2019spatial}. Please zoom in for a better view.}
  \label{fig:short}
\end{figure*}

==> sec/fig_tex/real/real-6.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/rainy_27.jpg}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/rainy_51.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/spdnet_27.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/spdnet_51.png}
  \end{subfigure}
    \subcaption[]{SPDNet}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/restormer_27.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/restormer_51.png}
  \end{subfigure}
    \subcaption[]{Restormer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/idt_27.jpg}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/idt_51.jpg}
  \end{subfigure}
    \subcaption[]{IDT}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/drsformer_27.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/drsformer_51.png}
  \end{subfigure}
    \subcaption[]{DRSformer}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/udr_27.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/udr_51.png}
  \end{subfigure}
    \subcaption[]{\scriptsize UDR-S$^2$Former}
    \end{minipage}
  \hfill
  \begin{minipage}{0.138\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/ours_27.png}
  \end{subfigure}
    \hfill
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/ours_51.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \caption{Visual comparisons of deraining on two samples from Internet-Data~\cite{wang2019spatial}. Please zoom in for a better view.}
  \label{fig:short}
\end{figure*}

==> sec/fig_tex/real/real-supple-1.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/rainy_69.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/dualgcn_69.png}
  \end{subfigure}
    \subcaption[]{DualGCN~\cite{Fu2021RainSR}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/spdnet_69.png}
  \end{subfigure}
    \subcaption[]{SPDNet~\cite{yi2021Structure}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/restormer_69.png}
  \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/idt_69.jpg}
  \end{subfigure}
    \subcaption[]{IDT~\cite{xiao2022image}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/drsformer_69.png}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{chen2023learning}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/udr_69.png}
  \end{subfigure}
    \subcaption[]{UDR-S$^2$Former~\cite{chen2023sparse}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/ours_69.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \caption{A visual comparison of deraining on Internet-Data~\cite{wang2019spatial}.}
  \label{fig:real-supple-1}
\end{figure*}

==> sec/fig_tex/real/real-supple-2.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.445\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/rainy_89.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.445\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/dualgcn_89.png}
  \end{subfigure}
    \subcaption[]{DualGCN~\cite{Fu2021RainSR}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.445\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/spdnet_89.png}
  \end{subfigure}
    \subcaption[]{SPDNet~\cite{yi2021Structure}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.445\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/restormer_89.png}
  \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.445\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/idt_89.jpg}
  \end{subfigure}
    \subcaption[]{IDT~\cite{xiao2022image}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.445\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/drsformer_89.png}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{chen2023learning}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.445\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/udr_89.png}
  \end{subfigure}
    \subcaption[]{UDR-S$^2$Former~\cite{chen2023sparse}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.445\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/ours_89.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
    \vspace{-2mm}
  \caption{A visual comparison of deraining on Internet-Data~\cite{wang2019spatial}.}
  \label{fig:real-supple-2}
\end{figure*}

==> sec/fig_tex/real/real-supple-3.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/rainy_106.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/dualgcn_106.png}
  \end{subfigure}
    \subcaption[]{DualGCN~\cite{Fu2021RainSR}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/spdnet_106.png}
  \end{subfigure}
    \subcaption[]{SPDNet~\cite{yi2021Structure}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/restormer_106.png}
  \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/idt_106.jpg}
  \end{subfigure}
    \subcaption[]{IDT~\cite{xiao2022image}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/drsformer_106.png}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{chen2023learning}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/udr_106.png}
  \end{subfigure}
    \subcaption[]{UDR-S$^2$Former~\cite{chen2023sparse}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/ours_106.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \caption{A visual comparison of deraining on Internet-Data~\cite{wang2019spatial}.}
  \label{fig:real-supple-3}
\end{figure*}

==> sec/fig_tex/real/real-supple-4.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/rainy_133.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hfill
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/dualgcn_133.png}
  \end{subfigure}
    \subcaption[]{DualGCN~\cite{Fu2021RainSR}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/spdnet_133.png}
  \end{subfigure}
    \subcaption[]{SPDNet~\cite{yi2021Structure}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/restormer_133.png}
  \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/idt_133.jpg}
  \end{subfigure}
    \subcaption[]{IDT~\cite{xiao2022image}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/drsformer_133.png}
  \end{subfigure}
    \subcaption[]{DRSformer~\cite{chen2023learning}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/udr_133.png}
  \end{subfigure}
    \subcaption[]{UDR-S$^2$Former~\cite{chen2023sparse}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.495\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{figs/real/ours_133.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \caption{A visual comparison of deraining on Internet-Data~\cite{wang2019spatial}.}
  \label{fig:real-supple-4}
\end{figure*}

==> sec/tab_tex/abla_five_table.tex <==
% \noindent
\begin{figure*}[!t]
\scriptsize
\renewcommand\arraystretch{1.}
\begin{minipage}{\linewidth}
\begin{minipage}[t]{0.194\linewidth}
\centering
\makeatletter\def\@captype{table}
\tabcolsep=0.5mm
    \caption{Ablation studies on the choice of the self-attention type.}\label{tab:abla_sa_type}%
    \vspace{-3mm}
    \begin{tabular}{lcc}
    \toprule
    Self-Attention & PSNR  & SSIM \\
    \midrule
    MDTA~\cite{zamir2022restormer}  & 32.37 & 0.9351 \\
    FSAS~\cite{kong2023efficient}  & 32.47 & 0.9364 \\
    TKSA~\cite{chen2023learning} & 32.54 & 0.9371 \\
    w/o SBR & 32.64 & 0.9383 \\
    SBSA  & \textbf{32.96} & \textbf{0.9409} \\
    \bottomrule
    \end{tabular}%
\end{minipage}
\hfill
\begin{minipage}[t]{0.194\linewidth}
\centering
\makeatletter\def\@captype{table}
\renewcommand\arraystretch{1}
\tabcolsep=1.2mm
    \caption{Ablation studies on the number of channels and bands.}\label{tab:abla_c_b}%
    \vspace{-3mm}
    \begin{tabular}{ccc}
    \toprule
    ($C_f,b$) & PSNR  & SSIM \\
    \midrule
    (72,1) & 32.74 & 0.9393 \\
    (36,2) & \textbf{32.96} & \textbf{0.9409} \\
    (18,4) & 32.78 & 0.9392 \\
    (9,8) & 32.33 & 0.9349 \\
    (4,18) & 31.72 & 0.9293\\
    \bottomrule
    \end{tabular}%
\end{minipage}
\hfill
\begin{minipage}[t]{0.194\linewidth}
\centering
\makeatletter\def\@captype{table}
\tabcolsep=0.5mm
    \caption{Ablation studies on feed-forward module}\label{tab:abla_ffn}%
    \vspace{-3mm}
    \begin{tabular}{lcc}
    \toprule
    Feed-Forward & PSNR  & SSIM \\
    \midrule
    FN~\cite{liang2021swinir}    & 32.47 & 0.9367 \\
    GDFN~\cite{zamir2022restormer}  & 32.58 & 0.9372 \\
    DFFN~\cite{kong2023efficient}  & 32.70 & 0.9384 \\
    MSFN~\cite{chen2023learning}  & 32.81 & 0.9391 \\
    SEFF  & \textbf{32.96} & \textbf{0.9409} \\
    \bottomrule
    \end{tabular}%
\end{minipage}
\hfill
\begin{minipage}[t]{0.194\linewidth}
\centering
\makeatletter\def\@captype{table}
\renewcommand\arraystretch{1}
\tabcolsep=0.5mm
  \caption{Ablation studies on state space module}\label{tab:abla_mamba}%
    \begin{tabular}{lcc}
    \toprule
    SSM & \multicolumn{1}{l}{PSNR} & \multicolumn{1}{l}{SSIM} \\
    \midrule
    VSSM~\cite{guo2024mambair} & 32.79 & 0.9388 \\
    For.+For. & 32.85 & 0.9402 \\
    Back.+Back. & 32.83 & 0.9399 \\
    Back.+For. & 32.94 & \textbf{0.941} \\
    For.+Back. & \textbf{32.96} & 0.9409 \\
    \bottomrule
    \end{tabular}%
\end{minipage}
\hfill
\begin{minipage}[t]{0.194\linewidth}
\centering
\makeatletter\def\@captype{table}
\renewcommand\arraystretch{0.89}
\tabcolsep=0.5mm
    \caption{Ablation studies on the setting of correlation loss}\label{tab:abla_cohloss}%
    \vspace{-3mm}
    \begin{tabular}{llcc}
    \toprule
          & $\alpha$ & PSNR  & SSIM \\
    \midrule
    w/o  $\mathcal{L}_{coh}$ & 0     & 32.75 & 0.9389 \\
    \midrule
    \multirow{4}{*}{w/ $\mathcal{L}_{coh}$} & 0.1   & 32.78 & 0.9394 \\
          & 1     & 32.86 & 0.9401 \\
          & 5     & \textbf{32.96} & \textbf{0.9409} \\
          & 10    & 32.85 & 0.9398 \\
    \bottomrule
    \end{tabular}%
\end{minipage}
\end{minipage}
\vspace{-2mm}
\end{figure*}



==> sec/tab_tex/abla_loss.tex <==
% \noindent
\begin{figure}[!t]
\footnotesize
\renewcommand\arraystretch{1.}
\begin{minipage}{\linewidth}
\begin{minipage}[t]{1.000\linewidth}
\centering
\makeatletter\def\@captype{table}
\renewcommand\arraystretch{0.89}
\tabcolsep=3mm
    \caption{Ablation studies on the setting of correlation loss}\label{tab:abla_cohloss}%
    % \vspace{-3mm}
    \begin{tabular}{llcc}
    \toprule
       Coherence Loss   & $\alpha$ & PSNR  & SSIM \\
    \midrule
    w/o  $\mathcal{L}_{coh}$ & 0     & 32.75 & 0.9389 \\
    \midrule
    \multirow{4}{*}{w/ $\mathcal{L}_{coh}$} & 0.1   & 32.78 & 0.9394 \\
          & 1     & 32.86 & 0.9401 \\
          & 5     & \textbf{32.96} & \textbf{0.9409} \\
          & 10    & 32.85 & 0.9398 \\
    \bottomrule
    \end{tabular}%
\end{minipage}
\end{minipage}
\vspace{-2mm}
\end{figure}



==> sec/tab_tex/complexity.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[htbp]
\footnotesize
\renewcommand\arraystretch{1}
\tabcolsep=1.mm
  \centering
  \caption{The performance evaluations of deraining methods encompassing PSNR, model size, computational complexity, and runtime are conducted. PSNR values are assessed on Rain200L~\cite{yang2017deep}, and FLOPs results are computed on input images of dimensions 256$\times$256. The values of runtime are tested on a Nvidia Tesla V100 GPU.}
  \vspace{-2mm}
    \begin{tabular}{lrrrrrrrrr}
    \toprule
          & \multicolumn{1}{l}{MSPFN~\cite{jiang2020multi}} & \multicolumn{1}{l}{MPRNet~\cite{zamir2021multi}} & \multicolumn{1}{l}{SPDNet~\cite{yi2021Structure}} & \multicolumn{1}{l}{Uformer~\cite{wang2022uformer}} & \multicolumn{1}{l}{Restormer~\cite{zamir2022restormer}} & \multicolumn{1}{l}{IDT~\cite{xiao2022image}} & \multicolumn{1}{l}{DRSformer~\cite{chen2023learning}} & \multicolumn{1}{l}{UDR-S$^2$Former~\cite{chen2023sparse}} & \multicolumn{1}{l}{SBFormer} \\
    \midrule
    PSNR & 38.58 & 39.47 & 40.50 & 40.20 & 40.99 & 40.74 & 41.23 & 40.96 & 41.56 \\
    % SSIM & 0.9827 & 0.9825 & 0.9875 & 0.9860 & 0.9890 & 0.9884 & 0.9894 & 0.9892 & 0.9938 \\
    \#Parameter & 21.00M & 3.64M & 3.32M & 20.63M & 26.10M & 16.42M & 33.70M & 8.53M & 15.68M \\
    FLOPs & 708.44G & 148.55G & 96.29 & 43.86G & 140.99G & 61.90G & 242.9G & 21.58G & 43.88G \\
    Runtime & 0.41 & 0.16 & 0.24 & 0.19  & 0.28  & 0.28  & 0.59  & 0.12 & 0.12 \\
    \bottomrule
    \end{tabular}%
  \label{tab:complexity}%
  \vspace{-2mm}
\end{table}%

==> sec/tab_tex/desnow.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[htbp]
\small
\renewcommand\arraystretch{0.6}
\tabcolsep=1.5mm
  \centering
  \caption{The metrics comparison of the deraining methods on Snow100K-L~\cite{liu2018desnownet}.}
  \vspace{-2mm}
    \begin{tabular}{lrrrrrr}
    \toprule
          & \multicolumn{1}{l}{MPRNet~\cite{zamir2021multi}} & \multicolumn{1}{l}{Restormer~\cite{zamir2022restormer}} & \multicolumn{1}{l}{IDT~\cite{xiao2022image}} & \multicolumn{1}{l}{DRSformer~\cite{chen2023learning}} & \multicolumn{1}{l}{UDR-S$^2$Former~\cite{chen2023sparse}} & \multicolumn{1}{l}{SBFormer} \\
    \midrule
    PSNR\(\uparrow\)  & 29.93  & 30.36  & 30.41  & 30.43  & 30.52  & \textbf{30.84} \\
    SSIM\(\uparrow\) & 0.9015 & 0.9068 & 0.9122 & 0.9143 & 0.9154 & \textbf{0.9228} \\
    \bottomrule
    \end{tabular}%
  \label{tab:desnow}%
  \vspace{-2mm}
\end{table}%


==> sec/tab_tex/desnow2.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[htbp]
\scriptsize
\renewcommand\arraystretch{0.6}
\tabcolsep=1.0mm
  \centering
  \caption{The metrics comparison of the deraining methods on Snow100K-L~\cite{liu2018desnownet}.}
  \vspace{-2mm}
    \begin{tabular}{lrrrrrr}
    \toprule
          & \multicolumn{1}{l}{MPRNet~\cite{zamir2021multi}} & \multicolumn{1}{l}{Restormer~\cite{zamir2022restormer}} & \multicolumn{1}{l}{IDT~\cite{xiao2022image}} & \multicolumn{1}{l}{DRSformer~\cite{chen2023learning}} & \multicolumn{1}{l}{UDR-S$^2$Former~\cite{chen2023sparse}} & \multicolumn{1}{l}{SDBFormer} \\
    \midrule
    PSNR\(\uparrow\)  & 29.93  & 30.36  & 30.41  & 30.43  & 30.52  & \textbf{30.84} \\
    SSIM\(\uparrow\) & 0.9015 & 0.9068 & 0.9122 & 0.9143 & 0.9154 & \textbf{0.9228} \\
    \bottomrule
    \end{tabular}%
  \label{tab:desnow}%
  \vspace{-2mm}
\end{table}%


==> sec/tab_tex/niqe.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[htbp]
\footnotesize
\renewcommand\arraystretch{1.}
\tabcolsep=1.2mm
  \centering
  \caption{The metrics comparison of real-world deraining involves non-reference image quality assessment on Internet-Data~\cite{wang2019spatial}.}
  \vspace{-2mm}
    \begin{tabular}{lrrrrrrrrrr}
    \toprule
          & \multicolumn{1}{l}{Rainy} & \multicolumn{1}{l}{MPRNet~\cite{zamir2021multi}} & \multicolumn{1}{l}{SPDNet~\cite{yi2021Structure}} & \multicolumn{1}{l}{Uformer~\cite{wang2022uformer}} & \multicolumn{1}{l}{Restormer~\cite{zamir2022restormer}} & \multicolumn{1}{l}{IDT~\cite{xiao2022image}} & \multicolumn{1}{l}{DRSformer~\cite{chen2023learning}} & \multicolumn{1}{l}{UDR-S$^2$Former~\cite{chen2023sparse}} & \multicolumn{1}{l}{SBFormer} \\
    \midrule
    NIQE\(\downarrow\)  & 3.66  & 4.14  & 3.88  & 4.21  & 3.62  & 3.71  & 4.03  & 3.52  & \textbf{3.40} \\
    BRISQUE\(\downarrow\) & 22.47 & 26.29 & 27.64 & 25.62 & 24.25 & 22.94 & 26.23 & 20.65 & \textbf{18.51} \\
    \bottomrule
    \end{tabular}%
  \label{tab:niqe}%
  \vspace{-2mm}
\end{table}%

